Lie Algebraic Cost Function Design for Control on Lie Groups

This paper presents a control framework on Lie groups by designing the control objective in its Lie algebra. Control on Lie groups is challenging due to its nonlinear nature and difficulties in system parameterization. Existing methods to design the control objective on a Lie group and then derive the gradient for controller design are non-trivial and can result in slow convergence in tracking control. We show that with a proper left-invariant metric, setting the gradient of the cost function as the tracking error in the Lie algebra leads to a quadratic Lyapunov function that enables globally exponential convergence. In the PD control case, we show that our controller can maintain an exponential convergence rate even when the initial error is approaching $\pi$ in SO(3). We also show the merit of this proposed framework in trajectory optimization. The proposed cost function enables the iterative Linear Quadratic Regulator (iLQR) to converge much faster than the Differential Dynamic Programming (DDP) with a well-adopted cost function when the initial trajectory is poorly initialized on SO(3).

==> draft.tex <==
\tsl{We will need to define the gradients in Riemannian geometry.}
Here we start with a tracking control problem of regulating the error between two trajectory. We refer to the definition of error function and velocity in \cite{bullo1999tracking}. Note that \cite{bullo1999tracking} considers the error function that enable us to consider the error trajectory. Thus assume the existence of the transport map that is compatible with the error function. 

We say that a function $h(\Psi)$ is an error function if it positive definite, such that $h(\Psi) \ge 0$ for any $\Psi$, and $h(\Psi) = 0$ if and only if $\Psi = I$. We also say that the error function is symmetry if $h(\Psi) = h(\Psi^{-1})$. 

Let $\mathrm{d}h(\Psi)$ denote the differential with respect to the $\Psi$. The error function $h(\Psi)$ is quadratic with constant if there exist two constants $0 \le b_1 \le b_2$, such that:
\begin{equation}
    b_1\|\mathrm{d}h(\Psi)\|_{M}^2 \le h(\Psi) \le b_1\|\mathrm{d}h(\Psi)\|_{M}^2, 
\end{equation}
where $\|\cdot\|_M$ is a norm induced by a metric. % \tsl{Needs more clarification? }. \tsl{For global property, we need to show that his unbounded in Lie Algebra.} 

For system on Lie Group, the velocity error is defined by the quantity:
\begin{equation}
    \dot{e}:=\xi - \mathrm{Ad}_{\Psi^{-1}}\xi_d
\end{equation}
Where $\mathrm{Ad}_{\Psi^{-1}}$ is the transport map that enabled the comparison between velocity in different reference frames.

Thus, the time derivative of an error function could be state as:
\begin{equation}
    \frac{d}{dt}h(\Psi)=\mathrm{d}h(\Psi)\cdot\dot{e}.
\end{equation}
\tsl{Designing the cost function h is hard. But we could shape the dh and show the existence of the corresponding h. }
% As there is a surjective mapping between the Lie Group elements and the corresponding Lie Algebra (in the normal branch of the logarithmic map), we replace $h(\Psi)$ with $h(\psi)$ as the error function. Now the derivative of the error function becomes $\mathrm{d}h(\psi)$, with is taken with respect to the Lie Algebra. 







% As the error function are defined on Lie Group, we

% \begin{equation}
%     \label{eq:error_grad}
%     \mathrm{d}\bar{h}(\Psi) = P\psi. 
% \end{equation}
% where $P$ is a positive definite matrix. 
% Then we have:
% \begin{equation}
% \begin{aligned}
%     \frac{d}{dt}\bar{h}(\Psi)&=\mathrm{d}\bar{h}(\Psi) \cdot \dot{e}\\
%     &=\psi^{\transpose}P\dot{e} \\
%     &=\psi^{\transpose}P({\xi - \mathrm{Ad}_{\Psi^{-1}}\xi_d}).
% \end{aligned}
% \end{equation}

% Thus, a control strategy is to design $\xi$ to enable the cost function decays with exponential rate. Thus, a trivial controller for the fist order system becomes:
% \begin{equation}
%     \xi = \mathrm{Ad}_{\Psi^{-1}}\xi_d - \psi. 
% \end{equation}
% Then have the closed loop system:
% \begin{equation}
%     \frac{d}{dt}\bar{h}(\Psi)=-\psi^{\transpose}P\psi. 
% \end{equation}
% Then, the remaining problem is to show the candidate error function $\bar{h}$ is an unbounded quadratic function with respect to $\psi$ given the gradient we designed in \eqref{eq:error_grad}. 


\begin{algorithm}[t]
\caption{Iterative Linear Quadratic Regulator on Lie Group}
\label{al:s_t_inference}
\begin{algorithmic}[1]
\State \textbf{Input:} Training data: $\mathcal{X}, \mathcal{Y}, \mathcal{Z}$; Query point: $x_\ast$
\State \textbf{Initialize:} semantic hyperparameters $\alpha_\ast^k \gets 0$
\State \hspace{1.45cm} traversability hyperparameters $\alpha_\ast, \beta_\ast \gets 0$ 
% \mgj{what's the difference between $\alpha_\ast^k$ and $\alpha^k$? I think these are semantic and traversability hyperparameters. Let's define them explicitly again.}
\For{each $(x_i, y_i) \in (\mathcal{X}, \mathcal{Y})$}
    \State $k_i \gets k(x_\ast, x_i)$
    \For{$k=1,...,K$}
        \State $\alpha_\ast^k \gets \alpha_\ast^k + k_i y_i^k$
    \EndFor
\EndFor \Comment{Semantic Mapping}
\For{each $(x_i, z_i) \in (\mathcal{X}, \mathcal{Z})$}
    \If{$x_i$ in cell $j$}
        \State $\alpha_j^\prime, \beta_j^\prime \gets 0$
        \For{$k=1,...,K$}
            \If{$k$th category is traversable}
                \State $\alpha_j^\prime \gets \alpha_j^\prime + \alpha_j^k$
            \ElsIf{$k$th category is untraversable}
                \State $\beta_j^\prime \gets \beta_j^\prime + \alpha_j^k$
            \EndIf
        \EndFor \Comment{Convert Dirichlet distribution to Beta}
        \State $\phi_j^\prime \gets (\alpha_j^\prime - 1) / (\alpha_j^\prime + \beta_j^\prime -2)$  \Comment{Compute mode}
        \State $u \sim \mathcal{U}(0, 1)$ \Comment{Draw a uniformly distributed random number}
        \If{$u \leq \phi_j^\prime$}
            \State $y_i^\prime \gets 1$
        \Else{}
            \State $y_i^\prime \gets 0$
        \EndIf \Comment{Sample from Bernoulli distribution}
    \EndIf
    \State $k_i \gets k(x_\ast, x_i)$
    \State $\alpha_\ast \gets \alpha_\ast + k_i (y_i^\prime + z_i)$ \Comment{Traversable posterior}
    \State $\beta_\ast \gets \beta_\ast + k_i (2 - y_i^\prime + z_i)$ \Comment{Untraversable posterior}
\EndFor \Comment{Semantic-Traversability Mapping}
\State \textbf{return} $\alpha_\ast^k, \alpha_\ast, \beta_\ast$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
Initialize with $Y_0=(X^0_{d,k}, \xi^0_{d,k}, u^0_{d,k}), k = 0, 1, 2, ..., N_t$.
\begin{algorithmic}[t]
\For{$n = 0, 1, 2, ..., N-1$}
\State Update the cost function in problem \eqref{prob:dtcmpc} based on $Y_n$. 
\State Solve problem \eqref{prob:dtcmpc} around the trajectory $Y_n$ to obtain the optimal policy $U=\{v_{ff, n}, K_{ff, n}\}$. 
\State Roll out the forward pass to obtain $Y_{n+1}$.  % $X^n_{d,k+1} = X^n_{d,k}\exp{(\xi_k\Delta t)}$
\EndFor
\Return $Y_{N}$
\end{algorithmic}
\end{algorithm}

==> method.tex <==
Supposing the input influence matrix $\mathcal{G}_k$ in output trajectory tracking control law \eqref{FTScontroller}  is unknown, we can formulate a constrained optimization problem to design the control input $u_k$ and the input influence matrix $\mathcal{G}_k$ concurrently. The finite-time stable tracking control law can be formulated as an equality constraints of a min norm controller:

\begin{equation}
    \begin{array}{c}
    \underset{\mathcal{G}_k, u_k}{\min} \|u_k\|_2^2 + w \|\mathcal{G}_k\|^2_{F} \\
    \mathcal{G}_k u_k=f_k \\
    % u_k \in \mathcal{U}, \mathcal{G}_k \in \mathcal{G} \\
    u_{\min} \le u_k \le u_{\max}, \\
    \|\mathcal{G}_{k} - \mathcal{G}_{k-1}\|_F\le L\|y_{k} - y_{k-1}\| \\
    sign(\mathcal{G}_{k}^{i,j})=s_{i,j}
    \end{array}
\end{equation}
where $w$ is a small positive weight to prevent $G_k$ from going to $0$. $u_{\min}$ and $u_{\max}$ are the lower and upper bounds of the control input. We also constrain the $\mathcal{G}_k$ to be Lipschitz continuous. Note that constraints on the sign of $\mathcal{G}_k$ is necessary. If we replace $\mathcal{G}_k$ with $-\mathcal{G}_k$, $-u_k$ then becomes the solution, which may not regulate the tracking error but amplifying it. 

TODO: We have to estimate the bounds of the tracking error here.
